StructComp: Substituting Propagation with Structural Compression in Training Graph Contrastive Learning

Graph contrastive learning (GCL) has become a powerful tool for learning graph data, but its scalability remains a significant challenge. In this work, we propose a simple yet effective training framework called Structural Compression (StructComp) to address this issue. Inspired by a sparse low-rank approximation on the diffusion matrix, StructComp trains the encoder with the compressed nodes. This allows the encoder not to perform any message passing during the training stage, and significantly reduces the number of sample pairs in the contrastive loss. We theoretically prove that the original GCL loss can be approximated with the contrastive loss computed by StructComp. Moreover, StructComp can be regarded as an additional regularization term for GCL models, resulting in a more robust encoder. Empirical studies on various datasets show that StructComp greatly reduces the time and memory consumption while improving model performance compared to the vanilla GCL models and scalable training methods.

==> remove.tex <==


\begin{table*}[!thbp]\small
	\caption{.}\label{tab:node}
	\centering
\begin{tabular}{lccc}\toprule
\multicolumn{1}{c}{\textbf{Method}}& \textbf{Cora} & \textbf{Citeseer}&\textbf{Pubmed}\\ 

\midrule
GS&81.5$\pm$0.8&71.2$\pm$1.0\\
JC&81.1$\pm$1.0&71.2$\pm$1.0\\
VN&81.3$\pm$0.9&71.3$\pm$1.0\\
METIS &81.6$\pm$0.9 &71.5$\pm$1.0&77.2$\pm$2.9\\
\midrule
GS\\
JC\\
VN\\
METIS&81.8$\pm$0.8&71.6$\pm$0.9&75.3$\pm$3.1\\
\midrule
GS\\
JC\\
VN\\
METIS&79.7$\pm$0.9 &70.5$\pm$1.0&77.2$\pm$1.4 \\
\midrule
GS& 78.7$\pm$0.9\\
JC\\
VN\\
METIS& 82.3$\pm$0.8&  71.6$\pm$0.9&78.3$\pm$2.5 \\
\bottomrule
\end{tabular}
\end{table*}
